A New Abstraction for Internet QoE Optimization

A perennial quest in networking research is how to achieve higher quality of experience (QoE) for users without incurring more resources. This work revisits an important yet often overlooked piece of the puzzle: what should the QoE abstraction be? A QoE abstraction is a representation of application quality that describes how decisions affect QoE. The conventional wisdom has relied on developing hand-crafted quality metrics (e.g., video rebuffering events, web page loading time) that are specialized to each application, content, and setting. We argue that in many cases, it maybe fundamentally hard to capture a user's perception of quality using a list of handcrafted metrics, and that expanding the metric list may lead to unnecessary complexity in the QoE model without a commensurate gain. Instead, we advocate for a new approach based on a new QoE abstraction called visual rendering. Rather than a list of metrics, we model the process of quality perception as a user watching a continuous "video" (visual rendering) of all the pixels on their screen. The key advantage of visual rendering is that it captures the full experience of a user with the same abstraction for all applications. This new abstraction opens new opportunities (e.g., the possibility of end-to-end deep learning models that infer QoE directly from a visual rendering) but it also gives rise to new research challenges (e.g., how to emulate the effect on visual rendering of an application decision). This paper makes the case for visual rendering as a unifying abstraction for Internet QoE and outlines a new research agenda to unleash its opportunities.

==> agenda.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US 


\section{Research agenda}

At this stage of our research, we do not yet know whether the advantages of \video will outweigh the challenges. 
In this section, we will decompose the challenges into individual topics that constitute the research agenda that
we are pursuing. 
We recognize our vision for re-architecting the QoE optimization frameworks is broader than what can be accomplished by us alone. 
By outlining a specific research agenda, we hope to spark discussions and efforts from the networking, multimedia and computer vision communities.

\subsection{\hspace{-0.3cm}From adaptation actions to \video}

\mypara{Accurate emulation}
The architecture in Figure~\ref{fig:framework} depends greatly on whether \video can be accurately emulated from adaptation actions. 
This is less of an obvious challenge in today's quality metric-centric approach, which needs to infer only the values of metrics, rather than the detailed rendering of a video or a web.
To this end, the adaptation protocol must be able to emulate the client-side behaviors, \eg when video player would stall if the bitrate is set in certain way and how the web browser would load and render the objects if they are prioritized in certain way. 

\jc{mention some web emulation tools (like Google Developers - Simulate Mobile Devices with Device Mode. \url{https:
//developers.google.com/web/tools/chrome-devtools/iterate/device-mode/}) and player emulation tools}

\mypara{Privacy concerns}
Besides the need for reconstructing more information, the \video inference raises concerns about user privacy too.
\jc{where to do it? client or server?}


\subsection{From \video to QoE}

\myparaq{What can be borrowed from computer vision}
Given the advances in computer vision, it is tempting to believe that we can borrow computer vision techniques, such as saliency detection or key moment detection, as alluded to by prior work~\cite{??,??}, to help develop \video-based QoE inference techniques.
However, we also recognize there are several mismatches between what these techniques are designed for and our goal. 
Specifically, many vision tasks focuses on what matters to information acquisition, rather than user experience of quality. This mismatch may be the reason for what we saw in Figure~\ref{fig:cv}.
\jc{add more discussion here}

\mypara{End-to-end training of QoE inference models}
Whether the QoE inference models will be built on existing vision models or from scratch, training such models will likely require large datasets of human-annotated \videos.
\jc{talk about mturk-based experiment}

\jc{also talk about possibility of transfer learning to customize them. }

\mypara{Overcoming limited compute power}
As \video retains more information than quality metrics, monitoring and optimization based on \video requires much more compute power, and in particular, this will be a limiting factor for energy constraint devices.
\jc{some discussion on moving most compute to the server or to precompute?}










%\task{Junchen to flesh out a first cut}
%
%\begin{itemize}
%
%\item how to infer visual rendering from adaptation actions
%\begin{itemize}
%\item challenges: (1) privacy, (2) how to know what happens on the client side (client may do local optimization)
%\item server-side emulation
%\item client-side instrumentation
%\end{itemize}
%
%\item how to build a qoe model based on visual rendering
%\begin{itemize}
%\item initial techniques from computer vision: saliency detection, highlight detection. 
%\item fundamental mismatches: 
%\begin{itemize}
%\item they are designed to capture what matters to information perception, not what matters to qoe. not taking into account how quality incidents affect user experience: need new dataset. solution: crowdsourcing?
%\item same model or separate models for different applications? solution: train a general model (common factors affecting qoe) and customize it per application
%\end{itemize}
%\end{itemize}
%
%\end{itemize}

==> arch.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US 

\section{Towards a new abstraction}


\subsection{Visual rendering}

Instead of developing more quality metrics, we explore a different approach.
We argue that QoE should be modeled not as a function of quality metrics, but directly from what a user visually sees on the screen. 
We call it a {\em \video}. 
Logically, it is represented as a (uncompressed) video recording of all pixels on the screen over time.
Figure~\ref{fig:framework} illustrates an example of a \video of a browser, in which it first loads a web page (search engine), then streams a video, and then loads another web page (news). 
Here, we assume the browser covers the full screen, but in general case, a \video might include multiple windows.


\mypara{\Video-driven QoE optimization}
Figure~\ref{fig:framework} depicts an end-to-end view of a \video-driven QoE-optimization framework. 
Logically the QoE optimization optimization involves two following key components.
For each potential adaptation action, 
\begin{packeditemize}
\item A {\em \video estimator} first infers the \video of the action, and then
\item A {\em \video-based QoE predictor} infers QoE of a given \video.
\end{packeditemize}
Finally, it can pick the action that achieves the best QoE.
In practice, this process can be sped up as discussed in \S\ref{??}.


\myparaq{What is captured (and not captured)}
{\em Intuitively, \video represents all visual input to the visual perception process that produces QoE.}
\video captures both the spatial experience (objects appearing on screen at the same time) as well as the temporal experience (dynamic loading of objects or playback of a video stream).
That said, \video does not include audio information (which is rarely integrated by QoE models, except those in acoustic literature), or contextual information, (\eg user device, individual users personal preference).


In short, QoE can be influenced by both visual factors and non-visual factors and \video could potentially entail all visual-related factors, but not non-visual factors.


\subsection{Advantages of \video}

Compared to quality metrics, \video as an abstraction for QoE modeling enjoys two unique advantages.


\myparashort{\#1: A unifying QoE abstraction.}
\Video is a unifying QoE abstraction that could capture QoE of both video and web applications.
For instance, it includes the frame-by-frame playback of a video streaming session as well as the sequence of object-loading events as seen by the user, from which prior quality metrics can be derived, including rebuffering time and page loading delay.\footnote{\Video alone does not capture metrics that require original content (\eg encoding quality of a video require the pixel values of the raw video), but it is possible to augment \video with the original content, just as prior QoE models.}


Moreover, \video could be used to derive QoE-determining factors that have not been considered yet.
%might affect potential future applications and adaptation actions.
For instance, in Figure~\ref{fig:cv}, the only difference between different ratings is the videos (with rebuffering at different positions) shown to the MTurkers, so \video should encode the hidden factors that causes the QoE difference (though we do not know what these hidden factors are yet).


From an architectural perspective, having a unifying abstraction for predicting QoE also stabilizes the ``interface'' between bandwidth-adaptive protocols and QoE prediction. 
In today's approach, when any new quality metric is added, the adaptive protocol needs to be updated to incorporate  the new metric and predict its value under each action.
In contrast, \video cleanly separate what adaptive protocol needs to monitor and estimate and how QoE is modeled.


%\Video includes information beyond a single application. 


%For instance, multi-party conferencing applications, such as Zoom or Hangout, have a different user interface than traditional Internet video
%users may perceive video quality differently than traditional 


%(\eg video streaming before and after full screen in Figure~\ref{fig:framework}) as well as temporal experience (\eg how fast first web session loads its page may subconsciously impact user's QoE expectation of the subsequent video web sessions).
%
%\Video encompasses all {\em visual} factors on the screen that might affect a user's experience. 
%\video captures both spatial experience (\eg video streaming before and after full screen in Figure~\ref{fig:framework}) as well as temporal experience (\eg how fast first web session loads its page may subconsciously impact user's QoE expectation of the subsequent video web sessions).
%
%\Video may {\em potentially} generalize to potential applications or adaptation actions. 
%
%
%\jc{new applications such as zoom, new actions such as slowing down videos, or even inter-application interactions (a youtube window shown side-by-side with a web browser)}


\myparashort{\#2: Enabling more accurate vision-based QoE models.}
The basic premise of \video is that it captures all visual input thus could potentially obtain more accurate QoE prediction. 
In particular, we envision training ``end-to-end'' model to predict QoE from \video.


Moreover, using \video as the input of QoE models opens up the possibility of building a unifying QoE model from which QoE models can be easily customized to various application settings.
The intuitive reason is that human visual perception follows the same biological procedures when watching videos or browsing web pages.\footnote{To be more precise, the visual perception processes do differ between passively browsing (\eg binge-watching videos) and actively thinking (\eg reading an important article), but such contrast is agnostic to the type of applications.}
This way, different application developers can significantly speed up the process to create their own QoE models 
(\eg different mobile web sites can derive their QoE models from the same basic model) rather than building each QoE model from scratch.


%\mypara{Technology ``pushes''}
We observe two favorable technical ``pushes'' that might enable this approach.
\begin{packeditemize}
\item {\em Alignment of computer vision and human vision:}
Deep neural networks (DNNs) achieve human-level (or better) performance on many tasks, especially vision-related tasks. This increasing alignment makes us hopeful that it is possible to train end-to-end DNNs to imitate QoE perception.
\item {\em Crowdsourcing platforms:}
Crowdsourcing platforms (\eg Amazon MTurk) lower the cost to create a large dataset of \videos annotated with QoE ``labels'', which can be used to train novel models that infers QoE from \videos.
\end{packeditemize}


%\mypara{2. Enabler of an unified QoE model}
%\jc{potential use of computer vision.. why a unifying qoe abstraction is even possible: human's visual perception follows the same biological procedure.}
%
%\Video not only applies to current adaptation actions but might apply to new adaptation actions as well.
%For instance, it is plausible for video streaming protocols to slow down the playback, rather than stalling, in order to replenish the video buffer.
%In today's approach, new quality metrics may be needed to capture model this new action's impact on QoE, but 


\subsection{Early promises from prior work}

The notion of \video does not exist in a vacuum.
We observe various form of this idea in some prior efforts.
Though they show early promises of \video, they do not push the concept to its logical extreme.

\mypara{Gaze tracking/prediction}
WebGaze~\cite{??} presents a user study on web QoE and reveals that QoE poorly correlates with traditional page load time metrics. 
Instead, web QoE is heavily influenced by the gaze trajectory, which largely follows a common pattern when viewing the same web page. 
In particular, WebGaze also shares the insight that gaze also varies with dynamic web loading process, so gaze is tracked while a web loading process is replayed.
Some follow-up work automatically derives user gaze from web content (\eg~\cite{??}) and similar techniques are also developed to detect attention from raw video in video streaming (\eg~\cite{??}).
That said, these efforts use attention, either measured or derived, as yet another input (to reweight web objects or video pixels/chunks) in the QoE model, thus can be bounded by the granularity of objects. 


\mypara{Eliciting QoE feedback} 
EYEORG~\cite{eyeorg} has used recorded videos as the same interface to elicit user rating (QoE) for video streaming and web services. 
They do so for the reason that users may have different network connectivities, so rather than letting them stream the videos or load web pages, they control what users see by letting them see pre-recorded videos of a video session or web page loading process.
We share with this work the use of recorded videos as a generic interface. However, EYEORG (and others~\cite{??,??}) still model QoE as a function of pre-determined quality metrics.
%\jc{similarity: use of video as a generic interface for both video and web; diff: still modeling qoe as function of quality metrics}


%\jc{similarity: gaze not captured by traditional PLT-style metrics; diff: still use attention as an intermediate feature}


\mypara{Subjective importance of content}
A recent work~\cite{sensei-anonymized-link} has similar observation as Figure~\ref{fig:cv} that bad quality incidents (\eg rebuffering) can have different impact on video QoE depending on the video content in which it occurs.
It also shows that such heterogeneous impact of quality on QoE often cannot be explained by existing quality metrics. 
However, rather than deriving such impact directly from \video, the work relies on crowsourcing platform to profile the relative impact of quality at each video chunk, which is arguably not as cheap and fast as an automatic model envisioned in this work.


%\jc{similarity: user temporal attention might be affected by unknown factors, diff: it shows naive use of vision is not enough either}

%\mypara{What is new in \video}
%\jc{visual rendering also captures potential impact on qoe by how quality incidents affects the content seen by the user}











%\subsection{Visual rendering}
%
%\task{Sid: please take a stab at it}
%
%\begin{itemize}
%\item what it is: a video of all pixels on the screen over time
%
%\item what it captures: the full experience of an application user, including everything on the screen concurrently (spatial experience) and the memory effect of things happened before the current application (temporal experience)
%what it doesn't capture: contextual information
%
%\item key advantage \#1: a unifying qoe abstraction that subsume all quality metrics as well as new applications and new actions and cross application effect. why a unifying qoe abstraction is even possible: human's visual perception follows the same biological procedure.
%
%\item key advantage \#2: potential of training ``end-to-end'' vision model to infer qoe from visual rendering.
%a useful analogy: vision research had been based on extraction of high-level features before the rise of end-to-end dnns.
%
%\item relationship with using original content as input: visual rendering also captures potential impact on qoe by how quality incidents affects the content seen by the user
%
%\end{itemize}

%\subsection{Initial promises from prior work}
%
%\begin{itemize}
%
%\item aruna's web qoe project based on gaze tracking \task{Junchen to flesh out a first cut}
%
%\item eyeorg \task{Xu: please take a stab at it}
%
%\item sensei \task{Xu: please take a stab at it}
%
%\end{itemize}

%\subsection{QoE optimization framework}
%
%
%\begin{itemize}
%\item the new architecture will be centered around visual rendering. Figure~\ref{fig:framework}
%
%\item two key components:
%\begin{itemize}
%\item how adaptation actions affect the visual rendering
%\item how visual rendering affects qoe
%\end{itemize}
%
%\item optimization process: protocol adaptation: for each action, what would be the visual rendering and how would that affect final qoe
%
%\end{itemize}



==> intro.tex <==


\section{Introduction}


An inflection point of Internet traffic is afoot, driven by a multitude of trends of Internet applications (web, video, etc)---more devices with large screens, more high-fidelity content, more interactive applications, and less patient users.
Emerging network technology (5G) are likely to spur more application traffic than mitigating network congestion in the wide-area networks.
In short, application traffic can soon overwhelm the Internet capacity.
There is an ever stronger need to raise quality of experience (QoE) using less network bandwidth.


The quest for better QoE-resource tradeoffs have spurred a substantial body of research in networking and multimedia communities.
However, the basic approach remains the same.
QoE is modeled as a function of a handful of {\em quality metrics}\footnote{These quality metrics are sometimes referred to by different names, including key quality/performance indicators (KQI/KPI), application-level quality of service (QoS), etc.} (as depicted in Figure~\ref{fig:abstraction}(a)), which can be objectively measured and predicted.
Prior work then focuses either
on (1) searching for the right quality metrics and building a {\em QoE model} that infers QoE from these quality metrics, or
on (2) designing {\em adaptive application protocols} to optimize QoE.
%Most recent work in Internet video (\eg avoiding rebuffering and raising bitrate) and web services (\eg cutting page load time) falls in these two categories.

\begin{figure}[t]
\centering
\includegraphics[width=1\columnwidth]{figs/abstraction.pdf}
\tightcaption{}
\label{fig:abstraction}
\end{figure}

%However, these quality metrics maybe too limiting to fully capture the enormously complex process of QoE perception.
%this traditional approach has several drawbacks, all resulting from the use of quality metrics as the abstraction of modeling QoE from application quality.
At a high level, these quality metrics act as an ``information bottleneck'' that distills QoE-determining factors to just a list of numbers, but this process may miss a lot of information that heavily affects user QoE.
%, but these numbers are often necessarily insufficient to capture QoE perception.
For instance, video viewers do not perceive video quality by simply counting how long each stall lasts; rather the perceived QoE depends on how the stalls (or other metrics) adversely affect user's perception of the content.
As we will elaborate in \S\ref{??}, the lack of granularity of these quality metrics also limits the potentials of QoE optimization and in response, many fine-grained quality metrics are proposed to  ``patch'' the QoE models, including both video streaming and web services, creating a complexity apocalypse.

%For instance, quality metrics that are shown to affect video QoE have grown remarkably in the last decade, including various ways to model the impact of when each bad-quality incident occurs on QoE perception \cite{??} and a multitude of pixel-level metrics to account for the impact of scene complexity and dynamics among other things \cite{??}.
%Moreover, new quality metrics are increasingly handcrafted for certain device types (laptop vs smartphone vs headset) \cite{??}, content types (short vs long, live vs. video-on-demand) \cite{??}, and user types \cite{??}.
%Similarly, web QoE has seen a surge of handcrafted quality metrics in recent years, including variations of page-loading time, including above-the-fold delay, time-to-first-byte, \fillme~\cite{??}, as well as memory effect across multiple page-loading events over time~\cite{??}.

Creating more piecemeal patches to QoE models might be insufficient and unsustainable.
The way users perceive QoE is fundamentally more complex than what a (potentially long) list of metric values can capture.
In the meantime, expanding the quality metric set means higher QoE model complexity (the ways these quality metrics affect QoE are rarely independent), new instruments to measure these quality metrics, as well as new application protocols to optimize these quality metrics.
Each new application may call for new QoE models too.



In this paper, we advocate for a new abstraction for QoE modeling which we called {\em \video}---a video stream that encompasses the time sequence of everything seen by a user on the screen, including video playback, sequence of object rendering of web pages, etc.
Figure~\ref{fig:abstraction} contrasts the traditional quality metrics with a \video.
Note that a \video is not the original content but how the content, after all the adaptation (compression, simplification, reordering, etc), is displaced on the screen as seen by the user.

The abstraction of \video enjoys three unique advantages over the traditional quality metric-based approach.
\begin{itemize}
\item \Video (in theory) entails the information needed to calculate all quality metrics used by prior QoE model (except contextual information such as user's personal preference), and is a unifying abstraction that potentially applies to all visual applications, including video streaming and web services.
\item \Video (essentially a multidimensional tensor) is amenable for advanced computer-vision techniques, including saliency detection. \jc{need more elaboration}
\end{itemize}
In the meantime, we observe a fortuitous confluence of technology trends that makes \video not as radical a change it may seem (\eg advances in computer vision and crowdsourcing platforms).
%For instance, advances in computer vision have given rise to deep learning models imitate human-level cognition in certain tasks.



In the remaining of the paper, we will make a case for \video as a much needed new abstraction that can not only help better model user-perception of Internet QoE, but inspire new opportunities for optimizing QoE and saving network bandwidth.

\jc{
useful link that shows per-page qoe modeling goes a long way!}
\url{https://link.springer.com/content/pdf/10.1007%2F978-3-319-76481-8_3.pdf}

%\task{Junchen to flesh out a first cut}
%
%
%
%\begin{itemize}
%\item to achieve higher qoe, internet applications require more network resources than available and the demand is growing fast $\longrightarrow$ need for better qoe-resource tradeoffs
%
%\item the literature has followed two directions: 
%(1) accurate qoe model (qoe = F(quality metrics)), and 
%(2) adaptive protocols to optimize quality metrics.
%$\longrightarrow$ high qoe requires that quality metrics sufficiently capture qoe
%
%\item however, it's fundamentally hard to capture the enormously complex process of qoe perception by these quality metrics (a list of numbers).
%
%\item although adding quality metrics does sometimes improve qoe (e.g., e2e, sensei, pano, klotski, etc) it also increases the system complexity (qoe modeling, quality monitoring, and adaptive protocol) and unlikely lead to a principled way of modeling qoe.
%
%\item instead of relying on quality metrics, we advocate for {\em visual rendering of the screen as seen by the user} as a better abstraction for qoe modeling. 
%
%
%
%\item two unique advantages:
%\begin{itemize}
%\item a unifying abstraction that potentially captures the {\em full experience of a user}, including existing quality metrics. more applications: zoom? 
%\item allows for end-to-end qoe modeling using computer vision techniques
%\end{itemize}
%
%\item this is not as difficult as it may seem: visual rendering is easy to annotate (crowdsource), though its still trickier to get \video from actions
%
%\item \video enables better separation between actions and qoe.
%
%\item this paper elaborate the case for applications' {\em visual rendering} as a more expressive, sustainable and principled qoe abstraction and outline the key research questions.
%
%\end{itemize}

==> motivate.tex <==



\section{Motivation}

\subsection{Growing demands of applications}

While network applications grow more diverse (notably Internet-of-thing applications), user-facing applications, including web services and various Internet video services, still dominate the Internet traffic.
We observe several trends that fuel a rapid growth of the traffic of these applications.
\begin{packeditemize}
\item {\em More content is encoded in higher fidelity} and streamed to larger screens.
The fraction of 4K videos on YouTube grows from \fillme\% to \fillme\% in mere \fillme years and in \fillme years, VR headsets will \jc{cite something from pano}.
\item {\em More applications emphasize interactivity} among large groups of users, rater than having clear data producers (\eg CDN) to allow data distribution at scale. \jc{a sentence on interactive live videos like twitch}
\item {\em Users are ever more impatient with low quality services.} \jc{cite something about 1 sec stall causes more damage to user experience in 2020 than 2010. similarly PLT deadline decreases from what to what}
\item Finally, there are simply {\em more concurrent active users}.
\end{packeditemize}

At the same time, network infrastructure grows as well, but at an uneven rate.
Broadband penetration in the US \jc{cite some nick's studies that show uneven access of networks across communities}
The disparity between demand to achieve high QoE and available network resource is vividly shown by emergency decisions made by large application providers.
\jc{cite news of netflix/youtube/hulu lowering quality}

In short, these trends underlie an increasing {\em need for better tradeoffs between QoE and network resources (bandwidth);} either achieving higher QoE with the same bandwidth or reduce bandwidth usage without hurting QoE (thus serving more users).






\subsection{Accurate QoE modeling is the key}

A substantial body of work has been dedicated to developing application and network protocols/logics that controls its {\em actions} to optimize quality under dynamic bandwidth and resource availability.
While predicting and optimally adapting to dynamic network resources is important, the potential room for improvement of these adaptive protocols is fundamentally {\em limited by the accuracy and granularity of QoE modeling} for three reasons.


\mypara{Balancing conflicting quality metrics}
In lack of real-time feedback on subjective QoE from users, adaptive protocols optimize a list of {\em potentially conflicting} quality metrics. 
For instance, video QoE is known to be highly correlated with higher average bitrate, less bitrate switches, less rebuffering (stalls), and low join time (start-up delay), but maximizing bitrate and minimizing join time are often conflicting objectives, especially for short videos, and when bandwidth varies a lot, minimizing bitrate switches must sacrifice either high average bitrate or less rebuffering.
% Moreover, the impact of these metrics on QoE varies across content, devices, and other contextual factors. 
If an adaptive protocol optimizes these metrics with an incorrect priority among them, it will likely yield suboptimal QoE even though the adaptation is optimal.


\mypara{Non-linear impact of quality metrics}
The relationships between quality metrics and QoE are seldom proportional. 
The intuitive reason is that users have limited cognitive capacity to perceive quality of application.
For instance, page-loading time (PLT) has a sigmoid-like relationship with QoE. 
When PLT is below (or higher than) some threshold, it will be too fast (slow) for users to perceive any improvement (reduction) of PLT; only when PLT value is in the middle will the reduction make significant impact on QoE.
Knowing when quality metrics have diminishing impact on QoE is critical to achieve high QoE with minimum networking resource.


\mypara{Limiting the granularity of actions}
The granularity of QoE modeling also affects the granularity of adaptive actions.
For instance, some recent studies have suggested that the impact of stalls on video QoE depends also on when rebuffering occurs, but in most video QoE models, QoE is affected by the percentage of total time of stalls and bitrate adaptive protocols designed to optimize such QoE models cannot avoid rebuffering at places when users are particularly sensitive to stalls, even though today's video streaming protocols could take such actions.





\subsection{Today's QoE modeling: Are we heading to a dead end?}

\mypara{The march of quality metrics} 
Today's approach to QoE modeling boils QoE down to a set of quality metrics and 
% Developing quality metrics to accurately predict QoE in various applications has been a central theme in the literature. 
the conventional wisdom has been that finer-grained quality metrics lead to more accurate QoE prediction and better QoE.
As a result, the list of quality metrics has been growing, with each new metric being inspired bh a new angle that is not covered by prior work.
To see how finer-grained metrics help, we consider three examples from recent work.
\begin{packeditemize}
\item {\em Example~\#1: User attention in \vr videos.} It is well known that \vr video viewers only pay attention to a small region (field of view or FoV) of the video at a time. 
While the original estimate of FoV is quite conservative (typically an area of \fillme$\times$\fillme), many recent work has dramatically refined it by taking into account various factors that might affect user perception (including the speed of the head movements, complexity of the scene, shape of objects, etc).
\item {\em Example~\#2: Impact of stalls of video QoE.} 
Video streaming QoE is affected by stalls and their impact was originally modeled by rebuffering ratio (the fraction of total duration of stalls in a video session), but over the years, this model has grown substantially more complicated in order to distinguish stalls occurring during dynamic scenes (which inflict more negative impact on QoE) and capture temporal patterns of between stalls (\ie memory effect), among other things. 
\item {\em Example~\#3: Object prioritization of web.} 
Our understanding of Web QoE has followed a similar trend of progressively finer-grained metrics. 
Although PLT is known to highly affect web QoE, the QoE model today is significantly more complex than the original threshold-based model. 
There have been various ways of modeling how a user perceive the page loading process, such as when the process visually starts and ends (\eg time to first byte), and how the loading order of different types of objects affects user perception, and the impact of screen size (\eg above-the-folder), etc.
\end{packeditemize}




% \jc{need a subsection here to elaborate that qoe perception more complex than most people think}



\mypara{A growing list with no end in sight}
Though it is tempting to add yet another quality metric to the list when a new factor is reveal to influence QoE, it obtains higher QoE accuracy often at the expense of high system complexity, which could cause problems in the long run.
\begin{packeditemize}
\item First, more complex QoE models often affects the adaptive protocols, which need to be redesigned to monitor more quality metrics and optimize the new QoE model.
This sometimes may not be a big problem (\eg calculation of rebuffering ratio naturally collects information of individual stalls), but often this requires significant redesign for the system (\eg recent \vr video streaming protocols requires object detection in the raw video). 
\item Second, as quality metrics are heavily tied to specific applications or adaptation actions, any new applications or new adaptation actions may require new quality metrics.
For instance, it will hardly be a surprise if a string of new quality metrics are developed for multi-party video conferencing tools (\eg Zoom) since they have a different interface than traditional Internet video (YouTube).
\item Third, there can be repetitive efforts among these QoE models. \jc{give an examples here}
\end{packeditemize}

An immediate consequence is that industry has largely ignored many useful quality metrics, and instead has focused on developing bandwidth adaptive techniques tailored for a few quality metrics, even though it limits the potential QoE improvement.




\begin{figure}[t]
      \begin{subfigure}[t]{0.48\linewidth}
         \includegraphics[width=1.0\linewidth]{figs/cv_lava.pdf}
        %  \caption{Lava}
        \caption{Lava}
      \end{subfigure}
      \hfill
      \begin{subfigure}[t]{0.48\linewidth}
         \includegraphics[width=1.0\linewidth]{figs/cv_tank.pdf}
        % \caption{Tank}
        \caption{Tank}
      \end{subfigure}
      \hfill
      \begin{subfigure}[t]{0.48\linewidth}
            \includegraphics[width=1.0\linewidth]{figs/cv_vlog.pdf}
            \caption{Animal}
      \end{subfigure}
      \hfill
        \begin{subfigure}[t]{0.48\linewidth}
            \includegraphics[width=1.0\linewidth]{figs/cv_soccer.pdf}
            \caption{Soccer2}
      \end{subfigure}
    \tightcaption{\task{This graph should be redrawn} An example of complex interaction between quality metrics and QoE. 
    In each graph, a rebuffering event occurs at different positions (x-axis) of the same video. 
    The dots are based on ratings of the same \fillme (randomly selected) Mechanic Turkers, so the difference among the impact of various rebuffering events is not a result of inter-user heterogeneity.
    We see that the the impact of the rebuffering event on QoE (blue) is at best only loosely correlated with dynamics of video content (red) or content-level importance (purple).}
    \label{fig:cv}
\end{figure}


\begin{figure*}[t]
\centering
\includegraphics[width=2\columnwidth]{figs/framework.pdf}
\tightcaption{An illustration of \video and how it would be used as part of the QoE optimization process. 
Two key components in this architecture are: 
the {\em \video estimator} that infers the \video of the action, and the {\em \video-based QoE predictor} that infers QoE of a given \video.
}
\label{fig:framework}
\end{figure*}


\myparashort{Yet, the list may still not be long enough!}
Not only does the current trend seem unsustainable, we also argue that this may not be sufficient either. 
The conventional wisdom that a user's QoE is dominantly affected by a few quality metrics has been proved far from correct. 
As shown in recent work~\cite{??,??}, one of the reasons why QoE perception is hard to model is that {\em human visual perception is an enormously complex process}.
It can be affected by many factors, including the content of a web page or video, viewing history of a user, concurrent activity at the peripheral of the application, etc. 

To see how (mysteriously) complex this process can be, Figure~\ref{fig:cv} shows the sensitivity of video QoE to a rebuffering happening at different position of a video. 
The blue line shows relative user rating with rebuffering over the rating without rebuffering (\ie the impact of a rebuffering event on QoE when it occurs at certain position of the video). 
Note that the dots are based on ratings of the same \fillme (randomly selected) Mechanic Turkers, so the difference among the impact of various rebuffering events is not a result of inter-user heterogeneity.
The red line shows the predicted rebuffering sensitivity predicted by a recent work under the premise that rebuffering hurts QoE more when the content is more dynamic. 
The purple line shows the relative content-wise importance of each chunk. 
We see that the the impact of the rebuffering event on QoE is at best only loosely correlated with dynamics of video content or content-level importance.



Before we move on, it is worth noting that the current tendency of fine-grained feature engineering is analogous to computer vision research in the pre-deep-learning era where a dramatic growth of highly-specialized high-level visual features are developed, only to be subsumed by the advent of end-to-end deep (convolutional) neural networks which is far more accurate and flexible.
Maybe it's time for networking community to take a cue from history!




%\subsection{Why QoE perception is hard to model}
%
%There has been much work to explain why QoE perception is hard to model~\cite{??,??}.
%One of the key reasons is that human visual perception is an enormously complex process.








% \subsection{Growing demands of applications}

% \task{Junchen to flesh out a first cut}

% \begin{itemize}
% \item internet application traffic counts for the bulk of internet traffic and it grows rapidly, driven by several factors: more high-fidelity content, more big screens, more interactive applications, more impatient users, etc

% \item network resources grow not as faster and grow unevenly

% \item these trends mean a strong need for better qoe-resource tradeoffs (higher qoe without more bandwidth, or less bandwidth without hurting qoe)

% \end{itemize}

%\subsection{Accurate QoE modeling is the key}
%
%\task{Junchen to flesh out a first cut}
%
%\begin{itemize}
%
%\item adaptive protocols are fundamentally limited by the accuracy/granularity of qoe modeling. (even if future network conditions can be perfectly predicted, one can't directly optimize qoe if the qoe modeling is inaccurate)
%
%\item potentially more actions
%
%\end{itemize}

%\subsection{March of quality metrics}
%
%\task{Xu: please take a stab at it}
%
%\begin{itemize}
%
%\item decades of research has produced more and more quality metrics without a principled framework. 
%
%\item a few examples of finer-grained modeling leading to better qoe: memory effect, pano, klotski
%
%\item qoe perception is too complex to be expressed by a list of quality metric values.
%
%\end{itemize}
